The unusual emission from PSR B1859+07 with FAST

We present simultaneous broad-band radio observations on the abnormal emission mode from PSR B1859$+$07 using the Five-hundred-meter Aperture Spherical radio Telescope (FAST). This pulsar shows peculiar emission phenomena, which are occasional shifts of emission to an early rotational phase and mode change of emission at the normal phase. We confirm all these three emission modes with our datasets, including the B (burst) and Q (quiet) modes of the non-shift pulses and the emission shift mode with a quasi-periodicity of 155 pulses. We also identify a new type of emission shift event, which has emission at the normal phase during the event. We studied polarisation properties of these emission modes in details, and found that they all have similar polarisation angle (PA) curve, indicating the emission of all these three modes are from the same emission height.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

